Human Evaluation of Procedural Knowledge Graph Extraction from Text with Large Language Models

Procedural Knowledge is the know-how expressed in the form of sequences of steps needed to perform some tasks. Procedures are usually described by means of natural language texts, such as recipes or maintenance manuals, possibly spread across different documents and systems, and their interpretation and subsequent execution is often left to the reader. Representing such procedures in a Knowledge Graph (KG) can be the basis to build digital tools to support those users who need to apply or execute them. In this paper, we leverage Large Language Model (LLM) capabilities and propose a prompt engineering approach to extract steps, actions, objects, equipment and temporal information from a textual procedure, in order to populate a Procedural KG according to a pre-defined ontology. We evaluate the KG extraction results by means of a user study, in order to qualitatively and quantitatively assess the perceived quality and usefulness of the LLM-extracted procedural knowledge. We show that LLMs can produce outputs of acceptable quality and we assess the subjective perception of AI by human evaluators.

==> sections/old-evaluation.tex <==
The human assessment of the LLM results was designed as two sequential, separate tasks: (T1) the manual annotation of the steps, actions and tools from a procedure, by following the same instructions and an example that were given to the LLM as prompts, and (T2) the evaluation of the LLM results (steps, actions, tools) from the same procedure. %, in a 1 to 10 rating
The first task allows us to understand behaviour, instruction interpretation and level of agreement of people in executing such a task, to compare with the LLM respective performance. %the results of a human and an LLM, and how they interpret the procedure extraction instructions. 
With the second task, we collected feedback to understand how correct and useful the LLM results are perceived by humans.
Each participant could provide open comments on each extracted step, and was asked to evaluate the instructions given in the prompt.
24 participants were randomly split into 3 groups (G1, G2, G3 from now on) of 8 users: 19 males and 5 females, 10 aged 20-29, 9 aged 30-39, 4 aged 40-49 and 1 aged more than 50. %the majority of them (42\%) in the 20-29 age range. 
They indicated a high familiarity with computer science (mean of 4.1 on a 1-5 scale) and average familiarity with LLMs (2.45 on the same scale).
Each group was given one of the 3 procedures used for the experiments reported in Section \ref{sec:meth-rel}. %\footnote{Group 1: \emph{Fix a rubbing door}; Group 2: \emph{Cook honey glazed parsnips}; Group 3: \emph{Plant a bare root tree}}.
In the following, we summarise and discuss the results of both tasks, that we qualitatively and quantitatively evaluated.

\subsection{Manual annotation of procedures}
\label{sec:manual-ann}
\noindent \textbf{Steps extraction.} The number of annotated steps varied quite a lot (variance of $\sim$9 in G1 and $\sim$5 in G2).
Some users keep coordinate sentences within the same step, others build more atomic steps.
In some cases, new steps, absent from the input procedure, were introduced. % (e.g. \enquote{Ask the help of another person before performing the next step}).
Finally, while some users report as steps the exact sentences from the textual procedure (as shown in the example accompanying the instructions), others tend to rephrase/integrate/summarise the text of the step, to make it clearer/briefer/more complete, based on their interpretation.
Based on these results, we can conclude that (i) understanding which are the \enquote{boundaries} of a step is not trivial (and the prompt instructions fail in giving a precise definition), and (ii) humans are prone to adjust the task based on what they consider more useful/reasonable, thus going beyond the instruction and using their creativity/reasoning.

\noindent \textbf{Tools extraction.} While the number of tools does not vary much within G1 and G3, the tools extracted by G2 go from 1 to 16. This is mainly due to the fact that some users considered the food in the recipe as tools, while others forgot some tools (e.g. only \emph{spoon}, excluding \emph{bowl} or \emph{roasting tray}). Considering that also the LLM failed in extracting a number of tools, and based on some comments by the users, we can say that it is important to include in the prompt/instructions a more specific definition of the class of entities to be extracted. 

\noindent \textbf{Actions extraction.} Also the number of identified actions was not constant (variance of $\sim$7 in G1, more than 4 in G2). 
This difference is an indicator of the ambiguity/difficulty also of this task: e.g., \enquote{Give them a little twist} resulted in either \emph{give}, \emph{twist}, or \emph{give a twist}; in \enquote{Use a stepladder to look at the top} the annotated action was either \emph{use}, or \emph{look (at)}, or both. Sometimes, the same user was not consistent in applying their extraction criteria, phenomenon that we also observed in the LLM.
Moreover, some actions are inferred/rephrased by the participants, e.g. \emph{wait} as  action to perform in the step \enquote{allow the tree to soak}.

\noindent \textbf{Difficulty and confidence.} Users were asked, on a 1-5 scale, if i) they found the annotation task easy, and their answer was between \emph{neutral} and \emph{somewhat easy} (average 3.5); and (ii) they were confident about their output's correctness, and again they were quite certain (average of 3.62/3.5/4.12, SD of 0.74/0.99/0.74 in G1/G2/G3). This outcome, together with the high variability of their annotations, confirms that PK extraction from text is far from being a trivial task.

%\textcolor{red}{non mettiamo qui due cose sulle risposte degli utenti alla fine dell'annotazione manuale? (e magari anche dei numeri seppur inventati sul tempo impiegato?}

\subsection{Human evaluation of LLM results}
The evaluators were then asked to rate each step, tool and action extracted by the LLM on a 1-10 scale. To compare their evaluations, we computed their inter-rater agreement using the  Krippendorff's alpha metrics.
Given that their manual annotations were quite different, it is not surprising that the level of agreement considering all scores on steps/tools/actions is very low, with $\alpha$ values of 0.25/0.55/0.21 in G1/G2/G3 (values of $\alpha$ < 0.667 are usually considered as not reliable). 
%Users tend to agree slightly more on tools extraction evaluation, specifically in G1 (0.43), while, as expected, the disagreement is higher for tools in G2 (the recipe).
Such disagreement is another evidence that knowledge extraction from unstructured procedures is a potentially ambiguous task for humans too, even when perceived as (somewhat) easy.

It is interesting also to note that the evaluators used the entire 1-10 scale of ratings in their assessment: while the maximum value on the scale means that the LLM proves to be an effective solution for PK extraction (also considering that, on average, the manual annotation task described in \ref{sec:manual-ann} took $\sim$18 minutes), the very low ratings used by some users mean that the LLM is still not  perceived as \enquote{good enough} to solve the problem in a fully automated way.

We also asked users to rate the prompt and possibly comment on how to improve it. The rating was medium-high (average of 7.75/8/8.35 on a 1-10 scale in G1/G2/G3, with SD of 1.28/1.3/1.18), but they provided quite interesting suggestions: they reported the need for a better definition of what a tool is (\enquote{something needed to perform the action or used during the action}) and what constitutes a step (\enquote{whether a step is defined by only one sentence or if there can be multiple sentences}); they also found the entire prompt too long and not immediate (\enquote{it is necessary to concentrate to understand well what it requires}, \enquote{the language should be more natural, less like a list of commands}), suggesting somehow that the LLM would require the same cognitive effort of a person.

% SCUSATEMI MA LA PARTE CHE SEGUE MI SEMBRA COMPLETAMENTE INUTILE...
%\noindent Let us make some examples. The step with more disagreement is \enquote{Make the honey glaze} from the recipe (G2): users that gave a high score annotated this as a step in T1, while the 3 users giving a low score consider it as an introductory sentence to the next steps. Instead, all G1 users agree that \enquote{Remove the tape} is a good step.
%As for the tools, users from G2 highly disagree on a step where some ingredients (butter, margarine) are extracted as tools by the LLM, as already discussed in \ref{sec:manual-ann}, while they all agree on the tool extracted from the step \enquote{If you do damage a few, nip them off with a \emph{pair of sterilized pruners}}.
%\enquote{Make the honey glaze} evaluation shows a high disagreement also in terms of actions extraction (\emph{make}), however, this is due to the fact that the users not considering this as a step give the same low score also to the extracted tools and actions. Instead, all G3 users agree that the actions extracted from 4 out of 7 steps are good. No step/tool/action shows a total agreement when it comes to bad scores.  





%We conducted three experimental campaigns, involving three separate groups, each of eight users, for the three examples given in REFERENCE
%In this study, we designed three Forms questionnaires for the evaluation of a procedural annotation experience through a guided survey.

%After a brief introduction to procedural knowledge and the aim of the work, the users were guided, with an example, through the process of manual annotation of steps, and corresponding actions and annotations, within a defined procedure in a given context (each experimental campaign refers to a procedure in a different context). 
%Once the annotation task is completed, the user is provided with an assessment questionnaire: the aim is to evaluate the annotation produced by the LLM system on the same procedure manually annotated by the user. After the visualisation and the check of, respectively, the prompt instruction provided to the LLM, the procedure text, and the output produced by the LLM, the user answers a set of punctual questions about the LLM output providing opinions, expressed in a 1 to 10 rating, respectively for 1) the correct extraction of the step, 2) the corresponding annotated actions, and 3) the tools extracted, if any. 
%For each step, the user can also provide further open-ended comments to better explain the ratings given. In the latter section of the questionnaire, the user expresses, in a 1 to 10 rating, his/her opinion about the overall step division performed by the automated annotation task. Then, the user expresses an opinion about the prompt instructions given to the LLM system, with the possibility to indicate suggestions to better clarify what task is required to be performed by the system.
 
%Finally, profiling data is collected for each user, including information about age, gender, familiarity with computer science and familiarity with LLMs.
%Explain the task given to the user, the number of users involved, etc. \\

% Quantitative comparison btw LLM results and user results (e.g. \# of steps, \# of tools, etc.) for each \\
% Qualitative comparison btw LLM results and user results (some examples of differences etc.)


% a livello di prompt, sembra evidente sia da GPT sia da utente umano, che il tool non è descritto bene, perché c'è chi include anche il cibo, chi no (indicandolo come errore quando lo fa GPT), e anche GPT non è consistente su questo
% questione delle sottoprocedure (es vedi Dominik) ci può stare, dato che abbiamo mischiato headlines e descriptions degli step, e a volte l'headline è più generale e nella description ti dice esattamente cosa devi fare

% prima campagna, interessante step 3 come caso d'uso sulle azioni (la maggior parte sono d'accordo)

% sui tools, interessante lo step dello stepladder nella prima campagna, e quello del container della terza campagna (sono praticamente tutti d'accordo)

% "use to remove" e casi simili: genera confusione su quali siano le azioni da aggiungere (anche se nell'esempio c'era proprio un caso così, e uno degli utenti lo segnala

==> sections/old-methodology-results.tex <==
%Extracting from a procedure the steps, the actions that each step prescribes to perform, and the tools, if any, that support the performing of such actions, involves some commonsense reasoning, which precedes the final output of the knowledge graph generation. 
%As demonstrated in \cite{wei2022-cot-reasoning}, and confirmed by our experiments, Chain-of-Thought (CoT) prompting -- that is decomposing a problem into intermediate steps (prompts) and solve each of them sequentially -- significantly improves the ability of LLMs to perform complex reasoning tasks, including commonsense. 
After multiple refinement iterations described before,
%\footnote{The initial versions of prompts that we refer to in this Section can be found at \footnote{\url{xxx}}}, 
we came up with a CoT prompting approach decomposed into 7 steps that build the final answer incrementally, as explained below and depicted in Figure \ref{fig:CoT}.
%\footnote{See Appendix \ref{sec:app-prompts} for the actual prompts that we designed.}.
All steps follow a one-shot learning approach, i.e. we provide the model with one example of the execution of the task within each prompt.
%The procedure referred to in such example\footnote{Available on GitHub: \url{XXX}} has been artificially built.
%, as a reference on the expected structure and content of the response. 
%As a driving example, we will use the WikiHow procedure involved in such prompt refinement process, that is \emph{Clean a flat panel monitor}.
We ask the LLM to provide outputs in JSON format at each step, leaving the RDF generation to the last step, because this approach allowed us to obtain more accurate and consistent data.


\begin{figure}[htb]
    \centering
    \caption{Illustration of the Chain of Prompt for Procedural KG extraction.}
    \includegraphics[width=\linewidth]{img/PK-CoT}
    \label{fig:CoT}
\vspace{\spaceunderfig}
\end{figure}

\noindent \textbf{P1: Extract initial list of steps from procedure.} 
We instruct the LLM to extract a list of steps from the text. In the prompt, we (i) assign a role to the LLM (\enquote{expert in information extraction}), (ii) give a brief definition of procedure\footnote{\enquote{A procedure consists of some steps that, if executed, contribute to achieve a goal.}} and step\footnote{\enquote{A step is an instruction that describes an action that someone needs to perform.}}, and (iii) provide an example that shows the extraction of both correct and incorrect steps from an example procedure. 
In the working example, while correctly identifying the name and beginning of the actual procedure, it still classifies as steps some sentences that do not describe an action to achieve the overall goal, such as \enquote{Use care around the monitor}. 
%The total number of steps is 19.

\noindent \textbf{P2: Self-evaluate the extracted steps.} 
In our experiments, we realized that leveraging the self-evaluation ability of LLMs (e.g. cf. \cite{ren2023-self-eval}) would improve its performance in understanding what is a step, distinguishing it from other sentences between steps (warnings, suggestions, tips, potential actions, negative instructions, precautions).
In this prompt, we ask the LLM to evaluate its initial list of steps, and classify them as correct/incorrect providing a rationale for its evaluation.
We also better explain what types of sentences' structures do not comply with our definition of step, and provide an example. % where we self-evaluate the steps we previously extracted from the example procedure in \emph{P1}.\\
%The LLM identifies 8 steps of the test procedure as incorrect. 
%The explanations are similar to the ones we provided in the example; however, i
It is interesting to notice that the LLM shows its reasoning capabilities in understanding how to provide a coherent explanation for each step. 
%For instance, the step we previously mentioned is identified as incorrect because \enquote{xxx}.

\noindent \textbf{P3: Discard incorrect steps.}
As a separate step, we ask the LLM to remove all steps identified as incorrect in \emph{P2}, so that we have our final list of steps. % (11 steps from our test procedure).

%\noindent \textbf{P1+P2+P3 engineering.} Initially, in place of this chain of prompts, a single prompt explained the whole task (including examples of sentences not to be considered as steps), directly showing the final list of steps from the example procedure. The LLM
%, while correctly ignoring some irrelevant sentences, 
%included 3 incorrect steps that were then discarded thanks to \emph{P2}: for example, \enquote{Use care around the monitor} has been identified as incorrect in \emph{P2} because \enquote{it is a general statement about being careful around the monitor}.

\noindent \textbf{P4: Number the steps.}
%The steps of a procedure need to be executed in an exact order. 
With this prompt, the LLM adds an incremental number to each step, following the structure of our example.

\noindent \textbf{P5: Extract tools from each step.}
At this point, we ask the LLM to analyse each step, and find the tools, intended as any kind of object that is needed to perform the step. We specify that it needs to include only the tools explicitly mentioned in the text, to try and avoid the LLM to infer some implicit/potential tools (e.g. \emph{shovel} for the action \emph{dig})\footnote{In this experiment, we want the LLM to strictly adhere to the source text; however, inferring implicit tools may be an interesting feature to explore.}. E.g., from \enquote{Use the cloth to wipe up smudges and fingerprints as needed}, the LLM extracts the \emph{cloth} tool. However, it missed the same tool from other steps.

\noindent \textbf{P6: Extract actions from each step.}
As a final extraction task, we ask the LLM to identify the action(s) included in each step. By action, we mean only the verb that corresponds to the task to be performed. In the prompt, we state that one step should contain at least one action. 
For instance, in the step \enquote{Purchase a soft cotton cleaning cloth for maintenance}, the extracted action is \emph{purchase}.
However, it is not trivial when it comes to phrasal verbs, e.g. the LLM reports only \emph{wipe} in place of \emph{wipe up}.
%non riesco più a fare un esempio di questo tipo con la nuova procedura (vd sotto)
%Moreover, it is not always consistent for the same sentence structure: for example, from \enquote{Use [...] to remove} extracts two actions (\emph{use}, \emph{remove}), while from the step \enquote{Use [...] to look} it extracts only \emph{use}. 

%\noindent \textbf{\textcolor{red}{Intermediate} output in JSON format.} At each step, the LLM stores its incremental output in a JSON format, with the same structure as the demonstrative example we provide. Thanks to its structure, inducing a JSON output allowed us to obtain more accurate and consistent data. 

\noindent \textbf{P7: Generate the knowledge graph of the procedure.} 
In order to obtain our final output -- that is a KG of the procedure, linked to its steps, actions and tools, according to an existing ontology -- we assign a new role to the LLM. \enquote{As an expert in linked data and knowledge engineering}, we ask it to follow the best practices of Linked Data and common standard vocabularies, as RDFS and OWL, for converting the procedure included in the JSON into an RDF KG formatted in Turtle syntax (similarly to \cite{frey_2023}). %The LLM is also asked to check the correctness of prefixes and syntax, and not to return additional text other than the Turtle triples.
%volendo, se avanza spazio, c'è il diagramma dell'ontologia nella cartella img, altrimenti solo su github e magari in appendice
Rather than providing the entire ontology to be used%\footnote{Example ontology (\texttt{po:}) covering experiment's requirements is on the GitHub repo.}
, we showed the language model an example translation from JSON to RDF, so that the LLM could find in the example all classes and properties to be used, and how they needed to be mapped to the JSON field names.
In Listing \ref{listing:llm-ttl-example}
%\footnote{po: <http://example.org/procedure-ontology\#>, ex: <http://example.org\#>} 
you can find the generated triples for the 10th step of our working procedure \enquote{Mix 1 part diluted isopropyl alcohol to 1 part water}.
\begin{lstlisting}[
    basicstyle=\ttfamily\scriptsize, frame=single, caption={Triples generated by the LLM from Step 10.}, label={listing:llm-ttl-example},mathescape] 
ex:CleanFlatPanelMonitor_step10 a po:Step ; 
rdfs:label "Mix 1 part diluted isopropyl alcohol 
            to 1 part water."^^rdfs:Literal ; 
po:isStepOf ex:CleanFlatPanelMonitor ; po:stepNumber "10"^^rdfs:Literal ; 
po:hasAction ex:Mix ; po:hasTool ex:DilutedIsopropylAlcohol , ex:Water ; 
po:hasNextStep ex:CleanFlatPanelMonitor_step11 ; 
po:hasPreviousStep ex:CleanFlatPanelMonitor_step9 . 
\end{lstlisting}

\noindent \textbf{About RDF generation.} 
While designing \emph{P7}, we started by providing the whole ontology, asking the LLM to translate its JSON output to Turtle according to such ontology.
However, relevant triples were missing: many inverse relations %, such as \texttt{po:hasNextStep} or \texttt{po:isToolOf}, 
were never used, and the procedure was linked only to the first step. Moreover, additional and very specific instructions would have been needed in the prompt for defining all prefixes and how to design local names, to prevent ambiguous individuals. %like \texttt{po:Action\_1}.
Instead, by showing by example how to map JSON to Turtle, we avoid possible errors in complying with ontological constraints,
%, such as domain and range restrictions on properties, 
with a greater guarantee of the final KG to be complete.
Moreover, this method may be particularly useful when we work with multiple, and possibly large, ontologies.

\noindent \textbf{Results.} After we tuned our CoT prompting approach on the first procedure, we run it on the other 3  procedures,  and again we manually evaluated the extracted information.
Table \ref{tab:procedures-stats} reports some statistics of the distinct entities (steps, tools, actions) extracted from the procedures, and the number of triples in the final RDF KGs. 
%As it can be noticed, ... se c'è spazio, aggiungere qualche commento sulle statistiche, per esempio il fatto che ci sono più azioni ripetute in rubbing door che nelle altre procedure, che in plant tree trova pochi tool 
%By manual inspection, we noticed that the LLM did not miss any sentence possibly representing a step from the procedure, except for the last step of the longest procedure. While all steps have at least one action, some actions are missing, and some sentences could have been split into multiple steps (as for \enquote{Warm the jar of honey in very hot water, then empty it into a bowl and stir in the butter or margarine}).
%In all procedures, the LLM struggled particularly in the tools extraction, which seems to be the most complex task: while it may indeed be ambiguous whether some objects are tools or not, based on our definition, it missed some obvious tools (e.g. \emph{pencil} in \enquote{Mark the door with a pencil}). 
%\\
%\emph{Procedural KGs evaluation.} 
All produced KGs are valid RDF in Turtle syntax. %\footnote{\url{http://ttl.summerofcode.be/}}. 
Properties' domains and ranges are correctly used, and individuals are typed flawlessly. The LLM perfectly mimics our conventions for local names.
%\textcolor{blue}{\\ cerca altre possibili metriche rilevanti}
%See paper on how well do LLMs speak turtle (mi pare) for other metrics (ma forse era un altro eh! quello dove passava l'onto verbalizzata

%completeness: did it missed some steps/actions/tools that was in the json? Did it missed some relations between subject/object?
% per questo, conta numero di tool azioni etc e confronta con numeri messi nella tabella sulla base dei json

\begin{table}[hb]
\centering
\caption{Statistics of the procedural KGs extracted by the LLM. } %\emph{P1} indicates the number of steps after the first prompt, \emph{P3} the final number of steps (with the number of errors in parentheses).}
\label{tab:procedures-stats}
	%\resizebox{.9\textwidth}{!}{ 
	%\begin{tabular}{p{2.1cm}|cc|c|c|c}
	\begin{tabular}{p{2.1cm}|c|c|c|c|c}
	\hline 
		%{ \bf Procedure} & \multicolumn{2}{c|}{{\bf \# steps}} & {\bf\# tools} & {\bf\# actions} & {\bf\# triples} \\\hline 
        % & P1 & P3 & & & \\  
		{ \bf Procedure} & {\bf steps after P1} & {\bf steps after P3} & {\bf tools} & {\bf actions} & {\bf total} \\
         & & { (removed steps)} & & & {\bf triples} \\
        \hline 
        \emph{Clean Monitor}  & 19 & 11 (8) & 4 & 10 & 136  \\
        \emph{Rubbing Door}  & 24 & 16 (8) & 7 & 14 & 204  \\
		\emph{Cook Parsnips}  & 16 & 14 (2) & 12 & 17 & 220 \\
        \emph{Plant Tree}  & 9 & 7 (2) & 3 & 8 & 94 \\		
%		\hline
	\end{tabular}
	%}
	\vspace{\spaceunderfig}
\end{table}


==> sections/old-motivating-example.tex <==
%Let us imagine a junior technician that is about to execute a maintenance procedure on a machine for the first time, and needs to consult the maintenance manual including all relevant information. Specifically, she needs to follow a sequence of steps, including actions to execute in a specific order; such actions may refer to relevant temporal information; she also needs to know which items are needed for performing the action (i.e., the equipment).
%Such technician may need an answer to the following questions:
\begin{itemize}
    \item Which are the steps of the procedure?
    \item Which is the step next to the one I have just executed?
    \item Which action do I need to perform in this step?
    \item Do I need some equipment for executing this step?
    \item Has the action to be executed a temporal duration to comply with?
\end{itemize}

==> sections/old-setting.tex <==
%-input data
%-che LLM usato
%-abbiamo fatto valutazione utenti per questo motivo etc more in section XX

%For our experiments, we used the GPT-3.5 Turbo model (gpt-3.5-turbo-16k version),
%\url{https://platform.openai.com/docs/models/gpt-3-5-turbo}
For our experiments, we used the GPT 4o model, and rely on the LangChain framework\footnote{\url{https://www.langchain.com/}}.
%, which simplifies the creation of LLM-based applications.
%, and allowed use to easily create and execute a chain of multiple prompts.
%In order to make the results as reproducible as possible, w
We set the temperature parameter to 0\footnote{Even with these settings, there is no guarantee that the result is always exactly the same. All results we refer to in this paper can be found on GitHub.}.
%, so that the highest probable next token is picked . 
%The results reported in this paper refer to a run on February 20th, 2024.}

\noindent \textbf{Input procedures.} We use as a reference WikiHow,
%\footnote{\url{https://wikihow.com/}}, 
one of the largest online databases of PK, which includes how-to articles on multiple domains. 
%WikiHow has been used in several past knowledge-base construction efforts (Pareti et al., 2014; Chu et al., 2017).
We reuse the JSON dataset built by \cite{zhang_reasoning_2020}, crawled from the WikiHow website\footnote{\url{https://github.com/zharry29/wikihow-goal-step}}, and focus on atomic procedures, that do not include methods/parts as sub-procedures.
%, which includes more than 110 thousand articles, crawled from the WikiHow website
Out of each selected procedure, we build an unformatted text (also partially removing punctuation), by concatenating  (i) procedure title, representing the overall goal, (ii) general procedure description, (iii) headline of each step, (iv) description of each step.
%aggiungi che abbiamo tolto parte della punteggiatura, che non ci sono indentazioni/a capo

%\noindent \textbf{\textcolor{red}{Evaluation}.} For the iterative prompt engineering process, we used a specific WikiHow procedure (see Section \ref{sec:meth-rel}), which is different from the procedures that have been randomly selected, from three different WikiHow categories, for the (human-based) validation, namely: Home Maintenance (\emph{How to fix a rubbing door}), Recipes (\emph{How to cook honey glazed parsnips}), and Gardening (\emph{How to plant a bare root tree}\footnote{This procedure has been partially truncated to prevent it from being much longer than the others.}).
%We do not take into account the WikiHow original step division as a reference for evaluation, since the steps' descriptions actually contain sentences that can be interpreted as steps in their own right.

% sotto "evaluation" qui io scriverei: quante procedure abbiamo usato (quali non è importante, sarà nella repo), come le abbiamo usate (provati i vari prompt su una e poi replicata sulle altre??), qual era il risultato atteso (una lista di step con azioni e tool, espressi in rdf secondo una data ontologia), e che in questa fase abbiamo valutato a mano i risultati confrontandoci tra noi per stabilire qualitativamente se il risultato fosse soddisfacente
\noindent \textbf{Evaluation.} In total, we used four procedures randomly selected from WikiHow, one as working example for our prompt engineering phase, and three for our method replication; the expected result for each procedure was a list sentences summarizing the steps extracted from the text, with their respective actions, direct objects and equipment items, expressed in RDF according to a given ontology; we manually evaluated the LLM results, finding an agreement between us with majority voting to decide whether each result was qualitatively satisfactory.

% dopo aver letto l'incipit della sezione successiva, forse anticiperei qui un'altra sottosezione "prompt engineering approach", in cui spiegherei che tentativi abbiamo fatto (zero shot, one shot, few shot, chain of thought), così poi nella sezione successiva c'è la nostra "soluzione"
\noindent \textbf{Prompt Engineering approach.} We tested different prompting approaches on the first procedure, to find the best solution; initially, we tried with a single prompt with zero/one/few-shot and we found that one prompt was not enough to achieve an acceptable result and a correct RDF, while giving one example in the prompt (one-shot learning) was the best trade-off; then, as demonstrated in \cite{wei2022-cot-reasoning}, we tried a Chain-of-Thought (CoT) prompting approach, i.e. decomposing the global problem into intermediate steps (prompts) and solve each of them sequentially, because this significantly improves the ability of LLMs to perform complex reasoning tasks,
including commonsense; we finally come up with a CoT prompting in 2 steps, as illustrated in the following.
